Minisuperspace computation of the Mabuchi spectrum

It was shown recently that, beside the traditional Liouville action, other functionals appear in the gravitational action of two-dimensional quantum gravity in the conformal gauge, the most important one being the Mabuchi functional. In a letter we proposed a minisuperspace action for this theory and used it to perform its canonical quantization. We found that the Hamiltonian of the Mabuchi theory is equal to the one of the Liouville theory and thus that the spectrum and correlation functions match in this approximation. In this paper we provide motivations to support our conjecture.

==> sections/flat_liouville.tex <==
\section{Comment on the flat Liouville theory}
\label{app:flat-liouville}


The flat (or BMS) Liouville theory corresponds to the asymptotic theory of $3d$ Minkowski $M_3$ in the same sense that the usual Liouville theory is the asymptotic theory of $\group{adS}_3$~\cite{Barnich:2012:FlatLimitThree, Barnich:2014:2DFieldTheory}.
Flat Liouville theory enjoys invariance under the infinite $\group{BMS}_3$ group which corresponds to the asymptotic symmetry group of $M_3$, in full parallel to Liouville theory which is invariant under Virasoro symmetry (the asymptotic symmetry of $\group{adS}_3$).
Since Minkowski spacetime can be seen as the limit of $\group{adS}$ for vanishing cosmological constant (or equivalently infinite cosmological length scale), it is expected that a similar limit can be used to obtain flat Liouville from Liouville.

In the minisuperspace approximation the Lagrangian of the flat Liouville theory is (we refer the reader to the literature for more details)
\begin{equation}
	L_{\text{flat}} = - 2\pi \mu\, \dot \varpi\, \Big[\ln \dot \varpi - 1 \Big].
\end{equation} 
This action corresponds to the potential of the Mabuchi action \eqref{mini:action:mabuchi} up to the identification
\begin{equation}
	\varpi = \frac{\ddot K}{8\pi \mu}.
\end{equation} 
This relation between the flat Liouville and Mabuchi theories should not be too surprising in view of \cref{sec:minisuperspace:deriv-legendre}.


